A Two-level Spatial In-Memory Index

Very large volumes of spatial data increasingly become available and demand effective management. While there has been decades of research on spatial data management, few works consider the current state of commodity hardware, having relatively large memory and the ability of parallel multi-core processing. In this work, we re-consider the design of spatial indexing under this new reality. Specifically, we propose a main-memory indexing approach for objects with spatial extent, which is based on a classic regular space partitioning into disjoint tiles. The novelty of our index is that the contents of each tile are further partitioned into four classes. This second-level partitioning not only reduces the number of comparisons required to compute the results, but also avoids the generation and elimination of duplicate results, which is an inherent problem of spatial indexes based on disjoint space partitioning. The spatial partitions defined by our indexing scheme are totally independent, facilitating effortless parallel evaluation, as no synchronization or communication between the partitions is necessary. We show how our index can be used to efficiently process spatial range queries and drastically reduce the cost of the refinement step of the queries. In addition, we study the efficient processing of numerous range queries in batch and in parallel. Extensive experiments on real datasets confirm the efficiency of our approaches.

==> sections/join.tex <==
\section{Spatial Join Evaluation}
\label{sec:join}
We next shift our focus to spatial joins. We discuss how our two-level
partitioning can be used to evaluate spatial intersection joins
efficiently, while avoiding the generation and elimination of
duplicate results.
We consider the problem of spatially joining two datasets
$R$ and $S$, which have both been partitioned using our two-level
partitioning sheme.
The two grids used for the partitioning are identical.
This means that we can apply the join phase of the PBSM algorithm
\cite{PatelD96} and apply a partition-to-partition join for each
pair of partitions from $R$ and $S$ that correspond to the same tile.

In details, given a spatial partition (tile) $T$, let $R_T$ and $S_T$ be the rectangles from
input dataset $R$ and $S$ that are assigned to $T$,
respectively.
$R_T$ is divided to rectangle groups $R^A_T$, $R^B_T$, $R^C_T$,
and $R^D_T$, according to our two-level partitioning scheme.
Similarly, $S_T$ is divided to $S^A_T$, $S^B_T$, $S^C_T$,
and $S^D_T$. Hence, the spatial join $R_T\bowtie S_T$ can now be
evaluated by 16 joins between smaller groups of rectangles,
i.e.,
$R^A_T \bowtie S^A_T, R^B_T \bowtie S^B_T, R^B_T \bowtie S^C_T, \dots, R^B_T \bowtie
S^A_T,\dots$. Figure \ref{fig:minijoins}  shows examples of join results for each of these group-group joins.


\begin{figure}[t]
\centering
  \includegraphics[width=0.99\columnwidth]{figures/mini-joins.pdf}
  \caption{Decomposition of tile $T$'s join into 16 joins.}
  \label{fig:minijoins}
\end{figure}

We can easily show that 7 out of these group-group joins (the shaded
cases in the figure) produce only duplicate results, i.e., join
results that will also be reported in another tile. For example, if two
rectangles of class $B$ in tile $T$ intersect (i.e., a result of
$R^B_T \bowtie S^B_T$),
then they will
definitely intersect also in another tile above $T$. 
We can also show that the remaining 9 group-group joins produce
only results that cannot be reported in any previous tile (in the $x$ or $y$
dimension or in both), but could be produced as duplicates in
some of the 7 shaded joins in a tile {\em after} $T$ in one or both
dimensions.
Hence, we {\em do not evaluate at all} the 7 shaded joins
and only evaluate the 9 group-group joins without performing any
duplicate elimination test.
%A subtle thing to note is that 

Each group-group join is evaluated using a
plane-sweep algorithm \cite{BrinkhoffKS93}
(alternative spatial join algorithms can also be used).
If the data are mostly static, we may pre-organize the contents of
each group by sorting them, e.g., based on their lowest value in the
first dimension.
When such a sorting already exists,
plane-sweep can be conducted even faster.
Keeping the contents of each group sorted can also accelerate range
queries as discussed in Section \ref{sec:range} (see Lemma \ref{lemma:comp1}).

Overall, our join algorithm replaces each tile-tile join by 9
smaller group-group joins. The result it produces is complete and
without duplicates.


==> sections/knn.tex <==
\section{kNN search}\label{sec:knn}

In this section, we show how our framework processes $k$NN queries.

$k$NN processing requires that we keep in a data structure (an array
or a hashmap) the number of rectangles that are assigned to each cell.
(For the moment, let us consider the filter step of the $k$NN query
only, or even better that the objects are points, which means that
there are no duplicates; for extended objects,
one could also consider the centers of the
objects only for measuring distances).
The data structure supports finding in $O(1)$ time the {\em number of
objects} that are assigned to a cell, given the cell's coordinates.

The $k$NN algorithm consists of the following steps:
\begin{itemize}
\item The coordinating thread (call it master or whatever) accesses
  the data structure to determine a set of {\em core cells} $C$.
  $C$ is defined as the {\em smallest set of cells} which are {\em the closest to
    the query point $q$} and collectively contain {\em at least $k$} objects.
  This set can be found by incremental search around $q$ (e.g., using
  Mouratidis' SIGMOD05 approach and ignoring empty cells).
  Let $d$ be the maximum of the maximum distances from $q$ to all
   cells in $C$. The $k$ nearest neighbor of $q$
   should have distance from $q$ at most $d$.
   Let $C'$ the set of cells which have distance at most $d$ from
   $q$, which includes $C$ and the set of {\em border cells} $C'-C$.
 \item
   the master asks all cells in $C'$ to compute in parallel the
   distances from $q$ to all objects in them. Loop-unroll to compute
   all these distances in parallel. Then, compute the local $k$NN at
   each cell and merge the results to get the global $k$NN set.
   Local $k$NN computation could even be skipped (we could simply
   aggregate {\em all} distances to get the $k$ smallest ones).
   For example, if a cell does not contain more than $k$ objects, it should just
   return all of them. In general, we should investigate here how to compute and
   rank these distances.  
% \item
%  use the $k$th distance to see whether more cells should be
%   examined. If a border cell (after the retrieved ones in $C$) has
%   min-distance smaller than the $k$th distance, ask it to compute its
%   local $k$NN. Gather all such local $k$NN results and merge them to
%   finalize the result. 
\end{itemize}
  
Figure \ref{fig:knnexample} illustrates and example for $k=50$.
The number on each cell corresponds to the number of objects assigned
to the cell. Assume for the moment that an object cannot be assigned
to more than one cells (i.e., there are no duplicates).
Duplicates can be handled by considering only some of the object
classes in each cell (to be investigated).
The orange/pink cells constitute the core set $C$, which is minimum
set of cells
which is the closest
to $q$ and contains at least $k$ objects. By taking the maximum
distance to any of these cells, we get a distance bound for the $k$-th
NN (shown by the line segment originating from $q$).
Using this bound, we can get all cells $C'$ (pink/orange + green ones)
that may contain the $k$NNs. Next, we compute the distances from all
objects in the cells $C'$ to $q$ and aggregate them to get the $k$NN
set. Investigate methods to do this efficiently and in parallel.
For some objects we could guarantee that they are in the $k$NN set
without any distance computations (for examples the objects in the
same cell as $q$).

\begin{figure}[htb]
\centering
  \includegraphics[width=0.89\columnwidth]{kNNexam.pdf}
  \caption{Example of $k$NN search ($k=50$)}
  \label{fig:knnexample}
\end{figure}

==> sections/preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelims}
We first introduce the necessary background in spatial data management \cite{2011Mamoulis}  for the rest of our paper. Specifically, we discuss basic spatial data and query types
and principles for query evaluation.

%\fix{define spatial data and queries; review the filter-refinement
%  framework; review classic spatial indexing prototypes; review recent
%  work that considers modern hardware} 

  
\subsection{Spatial Data and Queries}
\label{sec:prelims:queries}
Common types of spatial objects include points (defined by one value per dimension), rectangles (defined by one interval per dimension), line segments (defined by a pair of points), polygons (defined by a sequence of points), polylines (defined by a sequence of points), etc. 
%Figure 1(a) shows examples of these datatypes on the plane. 
%To characterize the relative position between two spatial objects,
To characterize the relative position and geometry between spatial objects, three classes of spatial relationships can be used.
\emph{Topological} relationships model the relation between the geometric extents of objects (e.g., overlap, inside).
\emph{Directional} relationships compare the relative locations of the objects with respect to a coordinate (or cardinal) system (e.g., north/south, above/below).
Last, \emph{distance} relationships capture distance/proximity information between two objects (e.g., near/far). 
%Figure 1(b) illustrates examples of spatial relationships.
%In this work, our focus is on query predicates defined with topological relationships for spatial objects with extent, e.g., rectangles and polygons; directional and distance-based predicates can also be easily handled and are left as future work.
The most frequently applied query operation on spatial data is the spatial \emph{selection} or \emph{range query} which retrieves the objects that for example intersect or are inside a well-defined area\eat{, or are within some distance from a reference object}. Formally:

\begin{definition}[Spatial Range Query]
Given a collection of objects $R$, a region $W$ and a predicate $\phi$, the \emph{spatial range} denoted by $\sigma_{\phi(\cdot,W)}(R)$ query returns all objects $r \in R$ that satisfy the $\phi(r,W)$ predicate.
\end{definition}
%\todo{Figure~\ref{} ...}

%Another common spatial query is the \emph{nearest neighbor}, which, given a well-defined reference object $q$, asks for the closest object to $q$ in space, with respect to distance measure, e.g., the Euclidean distance. Formally:
%\begin{definition}[Nearest Neighbor Query]
%Given a collection of objects $R$ and a reference object $q$, the \emph{nearest neighbor} query returns the object $r \in R$ such that for every $r' \in R \setminus \{r\}$,  $dist(q.r) \leq dist(q,r')$ holds.
%\end{definition}
%A straightforward extension to Definition~2 is to return the $k$ nearest neighbors of the query point $q$. \todo{Figure~\ref{}...}

Range \eat{and nearest-neighbor }queries are applied on a single spatial collection. The spatial join is a query that combines two collections, retrieving the subset of their Cartesian product that qualifies a given spatial predicate. Formally: 
\begin{definition}[Spatial Join Query]
Given two collections of objects $R$ and $S$, and a predicate $\phi$, the \emph{spatial join} query denoted by $R\bowtie_{\phi} S$, computes all pairs of objects $(r,s) \in R\times S$ that satisfy the $\phi(r, s)$ predicate.
\end{definition}
The most common join operation is the spatial \emph{intersection join} which returns all pairs of objects with overlapping geometries.
%\todo{Figure~\ref{}... }
%Other popular definitions of spatial joins include the $\epsilon$-distance join which determines $(r, s)$ pairs of objects within at most distance $\epsilon$ from each other, and the \emph{nearest-neighbor} join which returns for every object $r \in R$, the nearest objects from input $S$. 




\subsection{Query Processing Principles}
\label{sec:prelims:qprocess}
The potentially complex geometry of the objects renders inefficient the evaluation of spatial predicates directly on their exact representation.
\eat{
  For example, the cost of checking whether two polygons intersect is in the worst case $O(n\ log\ n)$, where $n$ is the total number of edges in the polygons. Therefore, to reduce the large computational overhead of spatial queries, a \emph{conservative} approximation is considered. The most common approximation is the \emph{Minimum Bounding Rectangle} (MBR), which is the smallest rectangle that encloses the geometry of an object.

\begin{figure}[t]
\centering
  \includegraphics[width=0.99\columnwidth]{figures/filter-refine.pdf}
%  \caption{The filtering-and-refinement approach for spatial query processing.}
	\caption{Two step query processing using object approximations (picture from \cite{2011Mamoulis}).}
  \label{fig:filter-refine}
\end{figure}
}
Hence, spatial queries are processed in two steps following a \emph{filtering-and-refinement} approach.
% \eat{, illustrated in Figure~\ref{fig:filter-refine}}.
During the \emph{filtering} step, the query is applied on
the \emph{Minimum Bounding Rectangles} (MBRs)
which approximate the objects.
If the MBR of the object (or the MBRs, in case of a spatial join) does not qualify the query predicate, then the exact geometry does not qualify it either.
%This can be demonstrated in Figure~\ref{fig:filter-refine}(b) where MBRs that do not intersect $W$ and so, do not enclose objects that qualify the query either.
The filtering step is a computationally cheap way to prune the search space, in many cases powered by spatial indexing, but it only provides candidate query results. During the \emph{refinement} step, the exact representations of the candidates are tested with the query predicate to retrieve the actual results.
%In Figure~\ref{fig:filter-refine}(c), observe that only two from the three candidates are query results.
In some cases, the refinement step can be avoided. For example, if at least one side of the MBR is inside the query range $W$, then the object definitely intersects $W$.

%spatial query evaluation is typically performed in two steps, also know as the \emph{filter-and-refinement} framework. In the filter step, the query is applied on the minimun bounding rectangles (MBRs) of the objects, which are simple lightweight approximations; see for example the MBR of a polygon in \todo{Figure~\ref{}}. Object MBRs (or pairs of object MBRs) that do not qualify the query can be pruned in the filter step, while for the objects (or object pairs) that pass the filter an expensive refinement step is applied using their exact geometries. For example, if the MBR of a river does not intersect the MBR of a city, there is no chance that the exact geometries of the two objects intersect.


 
% \subsection{Partitioning and Indexing}
% \label{sec:prelims:index}
